Set-based queries for multiscale shape-material modeling

Multiscale structures are becoming increasingly prevalent in the field of mechanical design. The variety of fine-scale structures and their respective representations results in an interoperability challenge. To address this, a query-based API was recently proposed which allows different representations to be combined across the scales for multiscale structures modeling. The query-based approach is fully parallelizable and has a low memory footprint; however, this architecture requires repeated evaluation of the fine-scale structures locally for each individual query. While this overhead is manageable for simpler fine-scale structures such as parametric lattice structures, it is problematic for structures requiring non-trivial computations, such as Voronoi foam structures. In this paper, we develop a set-based query that retains the compatibility and usability of the point-based query while leveraging locality between multiple point-based queries to provide a significant speedup and further decrease the memory consumption for common applications, including visualization and slicing for manufacturing planning. We first define the general set-based query that consolidates multiple point-based queries at arbitrary locations. We then implement specialized preprocessing methods for different types of fine-scale structures which are otherwise inefficient with the point-based query. Finally, we apply the set-based query to downstream applications such as ray-casting and slicing, increasing their performance by an order of magnitude. The overall improvements result in the generation and rendering of complex fine-scale structures such as Voronoi foams at interactive frame rates on the CPU.

==> sections/results_old.tex <==
\section{Results}
\label{sec:results}

\subsection{Testing Methodology}

% \x{include results for both single and multi thread, or put single thread result in Section 3?}

We run our tests on a consumer PC running an Intel i7 10700k CPU with 16 threads at 3.8 GHz and 64 GB of memory. While our approach may be extended to the GPU, for simplicity we choose to test it only with a CPU implementation. All timings are averaged over 3 runs and use wall time; detailed wall times for multithreaded tests are computed per-thread, and averaged across each thread.

We use several datasets for the performance testing of our program. We primarily use a 2-scale model with a coarse scale polygon model, and one finer scale. For the simple case, we use a simple cube for the coarse scale. We also use a 3D model of \todo{a femur and of a bracket} as additional coarse-scale models to show applicability to real-world use cases. For the fine scale, we either use a Unit Cell or a Voronoi Foam with a constant-space neighborhood grid of \todo{$32^3$, $256^3$, and $512^3$} cells.

We test the slicing application in both the single-core and multi-core context, running the membership query on a \todo{$545^3$, $1113^3$, and $2256^3$} grid of sample points. For the \todo{$2256^3$} grid, we also break the slicing apart such that only one Z-layer of the neighborhood grid is computed at once, simulating the case where the entire sample grid cannot fit in memory.

% For testing the general-use set queries, including the specializations on the Unit Cell and Voronoi Foam cases, we implement a slicing algorithm which simultaneously computes the membership query on a \todo{$545^3$, $1113^3$, and $2256^3$} grid of sample points. We also run an example where the \todo{$2256^3$} grid is broken up so only one Z-layer of the neighborhood grid is computed at once, to simulate the case where the entire sample grid cannot fit in memory.

We only test the ray set-query extension in the multicore case due to performance requirements. We also only test it on the Voronoi Foam microscale model. We sample a \todo{$256^2$, $1024^2$, and $2048^2$} image from \todo{two different angles, one in front of the model, and one from the corner} with both a regular ray-casting algorithm, and using our set-based query. For ray-casting, we use up to 3 steps per neighborhood grid cell, with the step length set to the distance query results according to sphere-tracing. The two methods differ only in how they sample the fine scale; sampling of the coarse scale is identical in both cases.

We also evaluate the performance of caching cells in the ray-tracing as explained in Section~\ref{sec:raycasting}. We use a simple first-in-first-out cache that stores the precomputed Voronoi edges with a maximum size of 1 GB.

\subsection{Single-core Results}

\begin{table}[!t]
\caption{Single-core Results.}
\label{tab:singleCore}
\centering
\begin{tabular}{|p{0.14\linewidth}| l| p{0.08\linewidth}| %p{0.06\linewidth}|
p{0.08\linewidth}|  %545
p{0.08\linewidth}|  %1113
p{0.08\linewidth}|  %2256
}
\hline
  Coarse Model & Fine Model & Grid Size & $545^3$ & $1113^3$ & $2256^3$ \\ \hline
\hline %     Fine       Neighbor   $545^3$  & $1113^3$ & $2256^3$
  Cube    & Unit Cell    &$16^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & Unit Cell    &$32^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & Unit Cell    &$64^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & V. Foam &$16^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & V. Foam &$32^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & V. Foam &$64^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Femur   & Unit Cell    &$16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & Unit Cell    &$32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & Unit Cell    &$64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & V. Foam &$16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & V. Foam &$32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & V. Foam &$64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & Unit Cell    &$16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & Unit Cell    &$32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & Unit Cell    &$64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & V. Foam &$16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & V. Foam &$32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & V. Foam &$64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
\end{tabular} 
\end{table}  
We show our single-core results in Table \ref{tab:singleCore}. We generally see a \todo{8x} improvement in performance over the point-by-point query, showing that our approach provides a significant performance improvement over the \naive{} case.

%<Detailed table of timings for a single test case - Unit Cell. Include column for per-point cost of regular method.>

%<Detailed table of timings for a single test case - Voronoi Foam. Include column for per-point cost of regular method.>

%We show the detailed timings for each phase of the algorithm in Tables \ref{tab:detailSC_UC} and \ref{tab:detailSC_VF}. 

For Unit Cells, the standard algorithm costs \todo{X}s per sample point. Our set-based query takes \todo{X}s per point to generate points, \todo{X}s for per-cell computations, and \todo{X}s of computation per sample point; this is a total of \todo{X}s per cell and \todo{X}s per point, meaning that we are faster than the \naive{} approach when there are at least \todo{X} points per cell. 

For Voronoi foams, the standard algorithm costs \todo{X}s per sample point. We take \todo{X}s per point for point generation, \todo{X}s per cell, and \todo{X}s per point of computation; this is a total cost of \todo{X}s per cell and \todo{X}s per point, meaning we are faster than the \naive{} approach when there are at least \todo{X} points per cell.

\subsection{Multi-core Results}

\begin{table}[!t]
\caption{Multi-core Results.}
\label{tab:multiCore}
\centering
\begin{tabular}{|p{0.14\linewidth}| l| p{0.08\linewidth}| %p{0.06\linewidth}|
p{0.08\linewidth}|  %545
p{0.08\linewidth}|  %1113
p{0.08\linewidth}|  %2256
}
\hline
  Coarse Model & Fine Model & Grid Size & $545^3$ & $1113^3$ & $2256^3$ \\ \hline
\hline %     Fine       Neighbor   $545^3$  & $1113^3$ & $2256^3$
  Cube    & Unit Cell    &$16^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & Unit Cell    &$32^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & Unit Cell    &$64^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & V. Foam &$16^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & V. Foam &$32^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & V. Foam &$64^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Femur   & Unit Cell    &$16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & Unit Cell    &$32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & Unit Cell    &$64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & V. Foam &$16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & V. Foam &$32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & V. Foam &$64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & Unit Cell    &$16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & Unit Cell    &$32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & Unit Cell    &$64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & V. Foam &$16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & V. Foam &$32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & V. Foam &$64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
\end{tabular} 
\end{table}  

We show our multi-core results in Table \ref{tab:multiCore}. We generally see a \todo{2x} improvement in performance over the point-by-point query; while this is less than our single-core performance gain, we still see a significant performance improvement.

%<Detailed table of timings for a single test case - Unit Cell. Include column for per-point cost of regular method.>

%<Detailed table of timings for a single test case - Voronoi Foam. Include column for per-point cost of regular method.>

%We show the detailed timings for each phase of the algorithm in Tables \ref{tab:detailMC_UC} and \ref{tab:detailMC_VF}. 

% The grouping cost is not easily multithreaded; our tests produced worse results when attempting to parallelize this task, likely due to excessive communications cost. See section \ref{sec:resultsConc} for more details.

For Unit Cells, the standard algorithm costs \todo{X}s per sample point. Our set-based query takes \todo{X}s per point to generate points, \todo{X}s for per-cell computations, and \todo{X}s of computation per sample point; we are faster than the \naive{} approach when there are at least \todo{X} points per cell. 

For Voronoi foams, the standard algorithm costs \todo{X}s per sample point. We take \todo{X}s per point for grouping, \todo{X}s per cell, and \todo{X}s per point of computation; we are faster than the \naive{} approach when there are at least \todo{X} points per cell.

\subsection{Ray Query Results}
\begin{table}[!t]
\caption{Rendering results.}
\label{tab:render}
\centering
\begin{tabular}{|p{0.14\linewidth}| l| p{0.08\linewidth}| %p{0.06\linewidth}|
r|  %256
r|  %1024
r|  %2048
}
\hline
  Coarse Model & Grid Size & $256^2$ & $1024^2$ & $2048^2$ \\ \hline
\hline %    Neighbor   $64^3$  & $1113^3$ & $2256^3$
  Cube    & $16^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & $32^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Cube    & $64^3$ & $0.00$s & $0.00$s & $0.15$s \\ \hline
  Femur   & $16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & $32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Femur   & $64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & $16^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & $32^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
  Bracket & $64^3$ & $0.00$s & $0.00$s & $0.82$s \\ \hline
\end{tabular} 
\end{table}  

We show our ray-query results in Table \ref{tab:render}. We can see that our approach offers an improvement over the standard case, providing a \todo{2x} speed improvement. 

We also see that the use of caching further provides a useful speed improvement when combined with our approach.

\todo{Insert table of detailed results}
%<Table of detailed results - VF>

\subsection{Conclusions}
\label{sec:resultsConc}

We found that in general, our approach offers a significant speed advantage over \naive{} point-by-point sampling. The more points need to be sampled per grid cell, the more efficient our approach is. \todo{Detailed explanation of scaling, if applicable.}

% Our major bottleneck is the inability to efficiently multithread the grouping of sample points; however, this bottleneck is only applicable when the sample points are assumed to be distributed arbitrarily. For cases where the sample points are aligned spatially or ordered in a regular fashion, we can implement far more efficient grouping algorithms which reduce or remove this cost.
